Improving Multimodal Learning with Multi-Loss Gradient Modulation

Learning from multiple modalities, such as audio and video, offers opportunities for leveraging complementary information, enhancing robustness, and improving contextual understanding and performance. However, combining such modalities presents challenges, especially when modalities differ in data structure, predictive contribution, and the complexity of their learning processes. It has been observed that one modality can potentially dominate the learning process, hindering the effective utilization of information from other modalities and leading to sub-optimal model performance. To address this issue the vast majority of previous works suggest to assess the unimodal contributions and dynamically adjust the training to equalize them. We improve upon previous work by introducing a multi-loss objective and further refining the balancing process, allowing it to dynamically adjust the learning pace of each modality in both directions, acceleration and deceleration, with the ability to phase out balancing effects upon convergence. We achieve superior results across three audio-video datasets: on CREMA-D, models with ResNet backbone encoders surpass the previous best by 1.9% to 12.4%, and Conformer backbone models deliver improvements ranging from 2.8% to 14.1% across different fusion methods. On AVE, improvements range from 2.7% to 7.7%, while on UCF101, gains reach up to 6.1%.

==> sec/2_modality_imbalance.tex <==

\section{Modality Imbalance}
\label{section:modality_imbalance}

In this section we aim to establish the intuition behind the problem. We show that gradients of a single joint multimodal objective are susceptible to modality competition, despite the network structure or fusion method employed.

We consider a classification task with a dataset $D$ of $N$ i.i.d. datapoints, where each datapoint has two modalities $(v, a)$. These modalities are expressed as sets of varying numbers of features with different statistical properties, denoted as $(X, y) = (x_i^v, x_i^a, y_i)$ for $i=1, \ldots, N$, where $x_i^v \in \mathbb{R}^{F^v}$, $x_i^a \in \mathbb{R}^{F^a}$, and $y_i \in {1, \ldots, M}$ with M representing the number of classes. The goal is to determine a parameterized function $f(X;\theta)$ to predict y. We consider models with a single output from both modalities. Such networks regardless of their fusion operation (early, mid, late, decision) can be cast as:
\begin{equation}
\label{eq:general_fusion_schema}
    f(X;\theta) = f^c(f^a(x^a; \theta^a)+f^v(x^v; \theta^v); \theta^c)
\end{equation}

As an illustration, if we choose to fuse on the decision level, then $f^c = \textbf{I}$, representing the identity matrix, where $c$ denotes the network that  combined in its input both modalities, and $\theta_c = \emptyset$. Alternatively, in the case of Late fusion, $f^c$ corresponds to a linear layer.  This general structure can also be seen in Figure \ref{fig:methods_sub3}. The $f^a$ and $f^v$ are the unimodal encoders with $\theta_a$ and $\theta_v$ being parameter dedicated respectively to each modality respectively. The dimensionality of the feature vectors produced by the unimodal encoders can vary in size $\phi^v = f^v(x^v; \theta^v)  \in \mathbb{R}^{\Phi_v}$ and $\phi^a =f^a(x^a; \theta^a) \in \mathbb{R}^{\Phi^a}$. 

We utilize two fusion examples: Late fusion with a linear classifier and Mid-Late fusion with a non-linear Multi-Layer Perceptron (MLP) classifier containing two hidden layers. For fusion, we use concatenation noted as $[\cdot, \cdot]$. For the two-layer MLP we use weights $\textbf{W}_1 \in \mathbb{R}^{\Phi^h \times (\Phi^v + \Phi^a)}$ with $\textbf{W}_1 = [ \textbf{W}_1^v,  \textbf{W}_1^a]$, $\textbf{W}_1^v\in \mathbb{R}^{\Phi^h \times \Phi^v}$,  $\textbf{W}_1^a \in \mathbb{R}^{\Phi^h \times \Phi^a}$, $b_1 \in \mathbb{R}^{\Phi^h}$, $\textbf{W}_2 \in \mathbb{R}^{M \times \Phi^h}$, $b_2 \in \mathbb{R}^{M}$ and  Rectified Linear Unit (ReLU) as the activation layer $\sigma$ to produce the logit outputs as follows:
\begin{align}
        f(\phi^v, \phi^a) &= \textbf{W}_2 \sigma(\textbf{W}_1 [\phi^v, \phi^a] + b_1)+b_2 \notag \\ &= \textbf{W}_2 \sigma(\textbf{W}_1^v \phi^v +  \textbf{W}_1^a \phi^a + b_1)+b_2 \notag \\ &= \textbf{W}_2 \sigma(g(\phi^v,\phi^a))+b_2
\end{align}

If our classifier was only a linear layer $g$ with $\Phi^h = M$ then the gradient of the loss with respect to $\textbf{W}_1^v$ would be:

\begin{equation}
\label{eq:grad_linear}
    \frac{\partial L}{\partial \textbf{W}_1^v}
    = \frac{\partial L}{\partial g(\phi^v, \phi^a)_{y_i}}
    \phi^v 
\end{equation}

While if we consider the classifier to be the function $f$, then using $\frac{\partial \sigma(x)}{\partial x}=z(x)=\{1 \text{ when } x>0 \text{, } 0 \text{ otherwise}\}$ the gradient would be:

\begin{align}
\label{eq:grad_nonlinear}
    \frac{\partial L}{\partial \textbf{W}_1^v} &= 
    \frac{\partial L}{\partial f(\phi^v, \phi^a)_{y_i}}
    \frac{\partial f(\phi^v, \phi^a)_{y_i}}{\partial\sigma(g(\phi^v, \phi^a))}\frac{\partial\sigma(g(\phi^v, \phi^a))}{\partial \textbf{W}_1^v} \notag \\
    &= \frac{\partial L}{\partial f(\phi^v, \phi^a)_{y_i}}
    w_{2_{y_i}}z(g(\phi^v, \phi^a))\phi^v
\end{align}
In our analysis, we found that modality $a$ significantly influences the gradient updates of weights $\textbf{W}_1^v$, which are specific to modality $v$. Determining the precise impact of each modality on these updates is not trivial. Contrary to our initial belief that more information sources would lead to faster convergence and a better local minima, the interaction between modalities can actually hinder performance. This is due to the phenomenon termed as Modality Competition \cite{huang2022modality}, where the more easily optimized modality suppresses the learning of others, potentially leading to sub-optimal learning outcomes.

In the nonlinear scenario, this dynamic becomes even more complicated, as the interaction between modalities deepens, potentially exacerbating their disruptive influence on each other. Our experiments, detailed in Section \ref{section:results}, empirically demonstrate this effect, showing greater suppression of one modality when integrated with an MLP classifier, as opposed to a linear model. 
